CryptoConcurrency: (Almost) Consensusless Asset Transfer with Shared Accounts

A typical blockchain protocol uses consensus to make sure that mutually mistrusting users agree on the order in which their operations on shared data are executed. However, it is known that asset transfer systems, by far the most popular application of blockchains, can be implemented without consensus. Assuming that no account can be accessed concurrently and every account belongs to a single owner, one can efficiently implement an asset transfer system in a purely asynchronous, consensus-free manner. It has also been shown that implementing asset transfer with shared accounts is impossible without consensus. In this paper, we propose CryptoConcurrency, an asset transfer protocol that allows concurrent accesses to be processed in parallel, without involving consensus, whenever possible. More precisely, if concurrent transfer operations on a given account do not lead to overspending, i.e. can all be applied without the account balance going below zero, they proceed in parallel. Otherwise, the account's owners may have to access an external consensus object. Notably, we avoid relying on a central, universally-trusted, consensus mechanism and allow each account to use its own consensus implementation, which only the owners of this account trust. This provides greater decentralization and flexibility.

==> sections/cryptographic-primitives.tex <==
\section{Cryptographic Primitives} \label{sec:crypto}

\myparagraph{Digital signatures}
We model digital signatures via an oracle, which provides the following functions:
\begin{itemize}
    \item $\fSign(m)$ -- returns a signature for message $m$;
    \item $\fVerify(m, \vSignature, p)$ returns $\True$ iff 
        $\vSignature$ was obtained with $\fSign(m)$ invoked by process $p$.
\end{itemize}

\myparagraph{Threshold signatures}

Additionally, we assume that $n-f$ valid signatures on the same message $m$ can be efficiently aggregated via a \emph{threshold signature scheme}~\cite{threshold-sig,boldyreva2003threshold} or a
\emph{multi-signature scheme}~\cite{ohta1999multi,boldyreva2003threshold}.
Namely, the following operations are available to all processes:
\begin{itemize}
        
    \item $\fCreateThresholdSignature(m, S)$ -- returns a threshold signature given a message $m$ and a set $S$ of valid digital signatures on message $m$ issued by $n-f$ distinct processes;

        
    \item $\fVerifyThresholdSignature(m, s)$ --  returns $\True$ iff signature $s$ was obtained by invoking $\fCreateThresholdSignature(m, S)$ for some set $S$.
\end{itemize}

\myparagraph{Merkle trees}



A Merkle tree (or a hash tree) is a binary tree in which every leaf node is labeled with a value (or a hash of a value) and every internal node is the hash of its two child nodes.
One can use it to efficiently create a short commitment (namely, the root of the tree) to a set of values $M = \{m_1, \ldots, m_k\}$.
Then, for any of the original values $m_i$, it is easy to prove that $m_i$ belongs to $M$ to somebody who only knows the root.
%
The proof simply consists of $\log_2 k$ sibling nodes of all nodes on the path from $m_i$ to the root in the tree.
%
We model this primitive with the below functions available to all processes:
\begin{itemize}
    \item $\fMerkleTree(ms)$ -- returns a Merkle tree $\vMerkleTree$ for the set of values $ms$. One can access the root of the tree using the notation $\vMerkleTree.\vMTRoot$;
    
    \item $\fGetItemProof(\vMerkleTree, m)$ -- returns a proof for item $m$ iff $\vMerkleTree = \fMerkleTree(ms)$ for some $ms$ such that $m \in ms$;
    
    \item $\fVerifyItemProof(\vMTRoot, \vItemProof, m)$ -- returns $\True$ iff $\vItemProof = \fGetItemProof(\vMerkleTree, m)$ for some $\vMerkleTree$ with $\vMerkleTree.\vMTRoot = \vMTRoot$.
\end{itemize}

In our protocols, Merkle tress could be replaced by more communication-efficient cryptographic primitives such as \emph{set accumulators}~\cite{set-accumulators} or \emph{vector commitments}~\cite{vector-commitments-1,vector-commitments-2}.
However, they typically require more expensive computation and a trusted setup.















